Multi-agent Natural Actor-critic Reinforcement Learning Algorithms

Multi-agent actor-critic algorithms are an important part of the Reinforcement Learning paradigm. We propose three fully decentralized multi-agent natural actor-critic (MAN) algorithms in this work. The objective is to collectively find a joint policy that maximizes the average long-term return of these agents. In the absence of a central controller and to preserve privacy, agents communicate some information to their neighbors via a time-varying communication network. We prove convergence of all the 3 MAN algorithms to a globally asymptotically stable set of the ODE corresponding to actor update; these use linear function approximations. We show that the Kullback-Leibler divergence between policies of successive iterates is proportional to the objective function's gradient. We observe that the minimum singular value of the Fisher information matrix is well within the reciprocal of the policy parameter dimension. Using this, we theoretically show that the optimal value of the deterministic variant of the MAN algorithm at each iterate dominates that of the standard gradient-based multi-agent actor-critic (MAAC) algorithm. To our knowledge, it is a first such result in multi-agent reinforcement learning (MARL). To illustrate the usefulness of our proposed algorithms, we implement them on a bi-lane traffic network to reduce the average network congestion. We observe an almost 25\% reduction in the average congestion in 2 MAN algorithms; the average congestion in another MAN algorithm is on par with the MAAC algorithm. We also consider a generic $15$ agent MARL; the performance of the MAN algorithms is again as good as the MAAC algorithm.

==> Other_tables.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|r|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Decision Epoch}} & \multicolumn{4}{c|}{\textbf{Arrival pattern 1}} & \multicolumn{4}{c|}{\textbf{Arrival pattern 2}} \\ \cline{2-9}
 & \textbf{MAAC} & \textbf{FI-MAN} & \multicolumn{1}{c|}{\textbf{AP-MAN}} & \textbf{FIAP-MAN} & \textbf{MAAC} & \textbf{FI-MAN} & \textbf{AP-MAN} & \textbf{FIAP-MAN} \\ \hline
\textbf{1300} & 10.07062 & 8.17687 & 10.08229 & 7.82611 & 10.12001 & 8.11726 & 10.13065 & 7.78031 \\ \hline
\textbf{1325} & 10.07405 & 8.16979 & 10.08569 & 7.82406 & 10.12350 & 8.11195 & 10.13358 & 7.77637 \\ \hline
\textbf{1350} & 10.06115 & 8.15568 & 10.07259 & 7.81535 & 10.12436 & 8.10156 & 10.13363 & 7.76481 \\ \hline
\textbf{1375} & 10.05710 & 8.14285 & 10.06829 & 7.80973 & 10.12537 & 8.09285 & 10.13474 & 7.75480 \\ \hline
\textbf{1400} & 10.05850 & 8.13102 & 10.07052 & 7.80447 & 10.12559 & 8.08654 & 10.13549 & 7.74760 \\ \hline
\textbf{1425} & 10.05437 & 8.11878 & 10.06620 & 7.79581 & 10.12375 & 8.07789 & 10.13295 & 7.73925 \\ \hline
\textbf{1450} & 10.05539 & 8.10304 & 10.06713 & 7.78483 & 10.12758 & 8.06486 & 10.13565 & 7.73017 \\ \hline
\textbf{1475} & 10.04889 & 8.08962 & 10.06165 & 7.77594 & 10.12046 & 8.05206 & 10.12870 & 7.71843 \\ \hline
\textbf{1500} & 10.05136 & 8.07926 & 10.06477 & 7.77147 & 10.11135 & 8.04344 & 10.12087 & 7.71313 \\ \hline
\end{tabular}
\caption{1500 decision epochs, 40000 vehicles. All values are averaged over 10 runs \textcolor{blue}{FI is doing significantly better, has  at least $20\%$ lower congestion than existing MAAC or the new first order and advantage fn based AP-MAN. At low congestion, FIAP does marginally better than FI (2nd decimal and in percentage terms it would be 3rd decimal, .001\% i think) but, it is marginally worse off at higher congestion.  Expectedly, both first order methods have reached steady state values; 2nd order one, FI almost (upto 1st decimal), but, is on decreasing trend w.r.t. congestion.}}
\end{table}
% \end{sideways}


\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|r|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Decision Epoch}} & \multicolumn{4}{c|}{\textbf{Arrival pattern 1}} & \multicolumn{4}{c|}{\textbf{Arrival pattern 2}} \\ \cline{2-9} 
 & \textbf{MAAC} & \textbf{FI-MAN} & \multicolumn{1}{c|}{\textbf{AP-MAN}} & \textbf{FIAP-MAN} & \textbf{MAAC} & \textbf{FI-MAN} & \textbf{AP-MAN} & \textbf{FIAP-MAN} \\ \hline
\textbf{1300} & 13.6579 & 10.26393 & 13.77954 & 10.29771 & 14.17963 & 10.34792 & 14.225 & 10.3476 \\ \hline
\textbf{1325} & 13.67816 & 10.25652 & 13.79778 & 10.29044 & 14.1847 & 10.33968 & 14.23449 & 10.3375 \\ \hline
\textbf{1350} & 13.66981 & 10.24446 & 13.7916 & 10.27473 & 14.17159 & 10.32218 & 14.22331 & 10.3154 \\ \hline
\textbf{1375} & 13.66056 & 10.231 & 13.78396 & 10.26192 & 14.17948 & 10.31042 & 14.22753 & 10.30083 \\ \hline
\textbf{1400} & 13.65649 & 10.21692 & 13.78262 & 10.24668 & 14.19757 & 10.30118 & 14.24721 & 10.29388 \\ \hline
\textbf{1425} & 13.66268 & 10.20342 & 13.78853 & 10.23542 & 14.20464 & 10.29229 & 14.25385 & 10.28777 \\ \hline
\textbf{1450} & 13.66189 & 10.19354 & 13.78971 & 10.22554 & 14.21093 & 10.27953 & 14.26026 & 10.27313 \\ \hline
\textbf{1475} & 13.64818 & 10.17327 & 13.77633 & 10.20473 & 14.2 & 10.26077 & 14.24961 & 10.25506 \\ \hline
\textbf{1500} & 13.64571 & 10.16988 & 13.77573 & 10.19858 & 14.20165 & 10.25633 & 14.25049 & 10.24845 \\ \hline
\end{tabular}
\caption{1500 decision epochs, 50000 vehicles. All values are averaged over 10 runs}
\end{table}

==> Tables-Traffic Light/Misc_Tables/50k-200_epochs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h!]
% \setlength{\tabcolsep}{2.5pt}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Algorithms} & \textbf{\begin{tabular}[c]{@{}c@{}}Decision \\ Epoch\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}Average\\  Congestion\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Standard\\Deviation\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Confidence Interval \\ (95\%)\end{tabular}} \\ \hline \hline
\multirow{5}{*}{\textbf{MAAC}} & 1300 & 14.04219 & 0.08587 & (13.98897, 14.09541) \\ \cline{2-5} 
 & 1350 & 14.03732 & 0.08768 & (13.98298, 14.09166) \\ \cline{2-5} 
 & 1400 & 14.03522 & 0.06993 & (13.99188, 14.07856) \\ \cline{2-5} 
 & 1450 & 14.03906 & 0.07464 & (13.99280, 14.08532) \\ \cline{2-5} 
 & 1500 & 14.01687 & 0.08405 & (13.96478, 14.06896) \\ \hline \hline
\multirow{5}{*}{\textbf{FI-MAN}} & 1300 & 12.12372 & 1.44496 & (11.22814, 13.01930) \\ \cline{2-5} 
 & 1350 & 12.10048 & 1.45755 & (11.19710, 13.00386) \\ \cline{2-5} 
 & 1400 & 12.08449 & 1.46756 & (11.17490, 12.99408) \\ \cline{2-5} 
 & 1450 & 12.06849 & 1.48525 & (11.14794, 12.98904) \\ \cline{2-5} 
 & 1500 & 12.02819 & 1.48071 & (11.11045, 12.94593) \\ \hline \hline
\multirow{5}{*}{\textbf{AP-MAN}} & 1300 & 14.09678 & 0.07737 & (14.04883, 14.14473) \\ \cline{2-5} 
 & 1350 & 14.08882 & 0.07551 & (14.04202, 14.13562) \\ \cline{2-5} 
 & 1400 & 14.09055 & 0.06271 & (14.05168, 14.12942) \\ \cline{2-5} 
 & 1450 & 14.09902 & 0.06632 & (14.05792, 14.14012) \\ \cline{2-5} 
 & 1500 & 14.07899 & 0.08266 & (14.02776, 14.13022) \\ \hline \hline
\multirow{5}{*}{\textbf{FIAP-MAN}} & 1300 & \textbf{11.47918} & 1.11561 & (10.78773, 12.17063) \\ \cline{2-5} 
 & 1350 & \textbf{11.42376} & 1.09733 & (10.74364, 12.10388) \\ \cline{2-5} 
 & 1400 & \textbf{11.38845} & 1.08963 & (10.71310, 12.06380) \\ \cline{2-5} 
 & 1450 & \textbf{11.34178} & 1.06876 & (10.67937, 12.00419) \\ \cline{2-5} 
 & 1500 & \textbf{11.28657} & 1.04137 & (10.64113, 11.93201) \\ \hline
\end{tabular}
\caption{For the arrival pattern 1, with $N_v = 50000$ table gives the average network congestion, standard deviation and 95\% confidence interval. The bold numbers are $\approx $ 18\% better than than MAAC and AP-MAN algorithms. \textcolor{blue}{we should try saying something like `congestion values within the top $15 \%$ are in bold'. also, this $15 \%$ should be used throughout the paper -- hopefully, it will work for other experiments also} Expectedly, both MAAC and AP-MAN have reached steady state values faster than other two algorithms. \textcolor{blue}{i wrote this earlier; not sure, if it is to be in caption; the point, is that FI-MAN would have lower congestion had it reached steady-state -- the way sumo works, we can't simulate this as 2000 decision epochs with same 50k vehicles is completely another system as these 50k are now placed uniformly over the 2000 epochs } FI-MAN and FIAP-MAN almost (upto 1st decimal) are on decreasing trend w.r.t. average network congestion however this decay is very slow (0.1 in 200 epochs). The performance of AP-MAN is almost similar to MAAC because it never uses the Fisher information matrix.}
\label{table: network_50K_pattern_1}
\end{table}

==> Tables-Traffic Light/Misc_Tables/50k-500_epochs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h!]
\centering
% \setlength{\tabcolsep}{2.5pt}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Algorithms} & \textbf{\begin{tabular}[c]{@{}c@{}}Decision \\ Epoch\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}Average\\  Congestion\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Standard\\Deviation\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Confidence Interval \\ (95\%)\end{tabular}} \\ \hline \hline
\multirow{5}{*}{\textbf{MAAC}} & 1300 & 13.65790 & 0.20956 & (13.52802, 13.78778) \\ \cline{2-5} 
 & 1350 & 13.66981 & 0.21010 & (13.53959, 13.80003) \\ \cline{2-5} 
 & 1400 & 13.65649 & 0.20735 & (13.52798, 13.78500) \\ \cline{2-5} 
 & 1450 & 13.66189 & 0.21023 & (13.53159, 13.79219) \\ \cline{2-5} 
 & 1500 & 13.64571 & 0.19755 & (13.52327, 13.76815) \\ \hline \hline
\multirow{5}{*}{\textbf{FI-MAN}} & 1300 & 10.26393 & 0.13996 & (10.17718, 10.35068) \\ \cline{2-5} 
 & 1350 & 10.24446 & 0.13366 & (10.16162, 10.32730) \\ \cline{2-5} 
 & 1400 & 10.21692 & 0.12768 & (10.13778, 10.29606) \\ \cline{2-5} 
 & 1450 & 10.19354 & 0.11760 & (10.12065, 10.26643) \\ \cline{2-5} 
 & 1500 & 10.16988 & 0.11877 & (10.09627, 10.24349) \\ \hline \hline
\multirow{5}{*}{\textbf{AP-MAN}} & 1300 & 13.77954 & 0.20823 & (13.65048, 13.90860) \\ \cline{2-5} 
 & 1350 & 13.79160 & 0.20285 & (13.66587, 13.91733) \\ \cline{2-5} 
 & 1400 & 13.78262 & 0.19888 & (13.65936, 13.90588) \\ \cline{2-5} 
 & 1450 & 13.78971 & 0.20300 & (13.66389, 13.91553) \\ \cline{2-5} 
 & 1500 & 13.77573 & 0.18925 & (13.65843, 13.89303) \\ \hline \hline
\multirow{5}{*}{\textbf{FIAP-MAN}} & 1300 & 10.29771 & 0.22585 & (10.15773, 10.43769) \\ \cline{2-5} 
 & 1350 & 10.27473 & 0.21690 & (10.14030, 10.40916) \\ \cline{2-5} 
 & 1400 & 10.24668 & 0.21714 & (10.11210, 10.38126) \\ \cline{2-5} 
 & 1450 & 10.22554 & 0.20637 & (10.09763, 10.35345) \\ \cline{2-5} 
 & 1500 & 10.19858 & 0.21248 & (10.06689, 10.33027) \\ \hline
\end{tabular}
\caption{For the arrival pattern 2 with $N_v = 50000$ table gives the average network congestion, standard deviation and 95\% confidence interval. The bold numbers are $\approx $ 25\% better than than MAAC and AP-MAN algorithms.  Expectedly, both MAAC and AP-MAN have reached steady state values faster than other two algorithms. FI-MAN and FIAP-MAN almost (upto 1st decimal) are on decreasing trend w.r.t. average network congestion however this decay is very slow (0.1 in 200 epochs). The performance of AP-MAN is almost similar to MAAC because it never uses the Fisher information matrix.}
\label{table: network_50K_pattern_2}
\end{table}

==> Tables-Traffic Light/Misc_Tables/50k_pattern_1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{lscape}
\begin{landscape}
\begin{table}[h!]
\centering
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Algorithms}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Decision \\ Epochs\end{tabular}}} & \multicolumn{2}{c|}{\textbf{$T_1$ Congestion}} & \multicolumn{2}{c|}{\textbf{$T_2$ Congestion}} & \multicolumn{2}{c|}{\textbf{$T_3$ Congestion}} & \multicolumn{2}{c|}{\textbf{$T_4$ Congestion}} & \multicolumn{3}{c|}{\textbf{Network Congestion}} \\ \cline{3-13}
 &  & \textbf{Average} & \textbf{CF} & \textbf{Average} & \textbf{CF} & \textbf{Average} & \textbf{CF} & \textbf{Average} & \textbf{CF} & \textbf{Average} & \textbf{Std Dvn} & \textbf{\begin{tabular}[c]{@{}c@{}}Confidence\\  Interval (95\%)\end{tabular}} \\ \hline
\multirow{5}{*}{\textbf{MAAC}} & 1300 & 3.48613 & 0.07369 & 3.37825 & 0.0314 & 3.34808 & 0.04214 & 3.44544 & 0.03706 & 13.6579 & 0.20956 & (13.52802, 13.78778) \\ \cline{2-13} 
 & 1350 & 3.48535 & 0.07283 & 3.37478 & 0.03094 & 3.36124 & 0.04133 & 3.44845 & 0.03451 & 13.66981 & 0.2101 & (13.53959, 13.80003) \\ \cline{2-13} 
 & 1400 & 3.48167 & 0.07123 & 3.37264 & 0.03411 & 3.35452 & 0.03959 & 3.44766 & 0.033 & 13.65649 & 0.20735 & (13.52798, 13.785) \\ \cline{2-13} 
 & 1450 & 3.48895 & 0.07275 & 3.3812 & 0.0347 & 3.34986 & 0.03445 & 3.44187 & 0.03648 & 13.66189 & 0.21023 & (13.53159, 13.79219) \\ \cline{2-13} 
 & 1500 & 3.48135 & 0.07022 & 3.3789 & 0.03437 & 3.34787 & 0.03225 & 3.4376 & 0.03317 & 13.64571 & 0.19755 & (13.52327, 13.76815) \\ \hline
\multirow{5}{*}{\textbf{FI-MAN}} & 1300 & 2.56024 & 0.0481 & 2.55406 & 0.04112 & 2.54095 & 0.04567 & 2.60867 & 0.0516 & 10.26393 & 0.13996 & (10.17718, 10.35068) \\ \cline{2-13} 
 & 1350 & 2.55422 & 0.047 & 2.54652 & 0.0442 & 2.53886 & 0.04525 & 2.60486 & 0.04825 & 10.24446 & 0.13366 & (10.16162, 10.3273) \\ \cline{2-13} 
 & 1400 & 2.5449 & 0.04746 & 2.53971 & 0.04345 & 2.53361 & 0.04357 & 2.5987 & 0.04685 & 10.21692 & 0.12768 & (10.13778, 10.29606) \\ \cline{2-13} 
 & 1450 & 2.54099 & 0.04608 & 2.53475 & 0.03961 & 2.52435 & 0.04443 & 2.59346 & 0.04546 & 10.19354 & 0.1176 & (10.12065, 10.26643) \\ \cline{2-13} 
 & 1500 & 2.53231 & 0.04671 & 2.52956 & 0.0403 & 2.51875 & 0.04505 & 2.58925 & 0.04524 & 10.16988 & 0.11877 & (10.09627, 10.24349) \\ \hline
\multirow{5}{*}{\textbf{AP-MAN}} & 1300 & 3.51468 & 0.07019 & 3.39959 & 0.02629 & 3.37735 & 0.04565 & 3.48793 & 0.03694 & 13.77954 & 0.20823 & (13.65048, 13.9086) \\ \cline{2-13} 
 & 1350 & 3.51448 & 0.06726 & 3.39834 & 0.02814 & 3.38832 & 0.04508 & 3.49046 & 0.03116 & 13.7916 & 0.20285 & (13.66587, 13.91733) \\ \cline{2-13} 
 & 1400 & 3.51273 & 0.06403 & 3.39686 & 0.03165 & 3.38276 & 0.04288 & 3.49027 & 0.02948 & 13.78262 & 0.19888 & (13.65936, 13.90588) \\ \cline{2-13} 
 & 1450 & 3.51785 & 0.06608 & 3.40663 & 0.0325 & 3.37742 & 0.03666 & 3.4878 & 0.0345 & 13.78971 & 0.203 & (13.66389, 13.91553) \\ \cline{2-13} 
 & 1500 & 3.51088 & 0.06365 & 3.40409 & 0.03187 & 3.37603 & 0.03398 & 3.48474 & 0.03319 & 13.77573 & 0.18925 & (13.65843, 13.89303) \\ \hline
\multirow{5}{*}{\textbf{FIAP-MAN}} & 1300 & 2.59067 & 0.043 & 2.55827 & 0.03719 & 2.56973 & 0.04291 & 2.57903 & 0.03786 & 10.29771 & 0.22585 & (10.15773, 10.43769) \\ \cline{2-13} 
 & 1350 & 2.58557 & 0.04211 & 2.54906 & 0.03567 & 2.56444 & 0.04254 & 2.57567 & 0.03408 & 10.27473 & 0.2169 & (10.1403, 10.40916) \\ \cline{2-13} 
 & 1400 & 2.57705 & 0.04227 & 2.54379 & 0.03481 & 2.55733 & 0.04124 & 2.56851 & 0.03504 & 10.24668 & 0.21714 & (10.1121, 10.38126) \\ \cline{2-13} 
 & 1450 & 2.57375 & 0.03922 & 2.54031 & 0.03352 & 2.54917 & 0.0408 & 2.5623 & 0.03431 & 10.22554 & 0.20637 & (10.09763, 10.35345) \\ \cline{2-13} 
 & 1500 & 2.5661 & 0.04086 & 2.53445 & 0.03377 & 2.54253 & 0.04141 & 2.5555 & 0.03583 & 10.19858 & 0.21248 & (10.06689, 10.33027) \\ \hline
\end{tabular}
\caption{50K arrival pattern 2}
\label{table: 5K_arrival_2}
\end{table}
\end{landscape}

==> Tables-Traffic Light/Misc_Tables/T-source_prob-prev.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h!]
\centering
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Source node \\ $(s)$\end{tabular}}} & \multicolumn{3}{c|}{\textbf{Arrival Pattern $(m)$}} \\ \cline{2-4} 
 & \textbf{$m=1$} & \textbf{$m=2$} & \textbf{$m=2^{\prime}$} \\ \hline \hline
$W_1$ & $\frac{3}{16}$ & $\frac{1}{28}$ & $\frac{3}{14}$ \\ \hline
$W_2$ & $\frac{1}{16}$ & $\frac{1}{28}$ & $\frac{3}{14}$ \\ \hline
$N_1$ & $\frac{1}{16}$ & $\frac{3}{14}$ & $\frac{1}{28}$ \\ \hline
$N_2$ & $\frac{3}{16}$ & $\frac{3}{14}$ & $\frac{1}{28}$ \\ \hline
$E_1$ & $\frac{3}{16}$ & $\frac{1}{28}$ & $\frac{3}{14}$ \\ \hline
$E_2$ & $\frac{1}{16}$ & $\frac{1}{28}$ & $\frac{3}{14}$ \\ \hline
$S_1$ & $\frac{1}{16}$ & $\frac{3}{14}$ & $\frac{1}{28}$ \\ \hline
$S_2$ & $\frac{3}{16}$ & $\frac{3}{14}$ & $\frac{1}{28}$ \\ \hline
\end{tabular}
\caption{Probability $p_{s,m}$ for all the nodes and arrival patterns. $m=1$ assigns high probabilities to a north and a south node, $N_2,S_2$ and to a east and a west nodes, $E_1,W_1$. $m=2$ assigns high probabilities to all north and south nodes, $N_1,S_1,N_2,S_2$.  $m=2^{\prime}$ which is symmetric to $m=2$ assigns high probability to all east and west nodes, $E_1,E_2,W_1,W_2$.}
\label{table: prob_source node}
\end{table}

% one North-South, i.e., $N_2, S_2$ and one East-West, i.e., $E_1, W_1$ nodes with higher probabilities, thus putting highest congestion on traffic light $T_2$, almost equal congestion on $T_1,T_4$ and the least congestion on $T_3$. However, for $m=2$ all North-South nodes have high probability and all East-West nodes have low probability. Thus we expect that all the traffic lights will have almost the same congestion. $m=2^{\prime}$ is symmetric to $m=2$ and hence more vehicles will be assigned to East-West nodes.

==> Tables-Traffic Light/Misc_Tables/T-source_prob_horizontal.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{Source Node (s)} & $W_1$ & $W_2$ & $N_1$ & $N_2$ & $E_1$ & $E_2$ & $S_1$ & $S_2$ \\ \hline
\textbf{ap} 1 \textbf{probability} & $3/16$ & $1/16$ & $1/16$ & $3/16$ & $3/16$ & $1/16$ & $1/16$ & $3/16$ \\ \hline
\textbf{ap} 2 \textbf{probability} & $1/28$ & $1/28$ & $3/14$ & $3/14$ & $1/28$ & $1/28$ & $3/14$ & $3/14$ \\ \hline
\end{tabular}
\caption{Probability $p_{s,ap}$ for source node $s$ and arrival pattern $ap$. $ap=1$ assigns high probability to $N_2,S_2$ and $E_1,W_1$ whereas, $ap=2$ assigns high probability to all north and south nodes $N_1,S_1,N_2,S_2$ in Figure \ref{fig: traffic_network}.}
\label{table: prob_source node}
\end{table}

==> Tables-Traffic Light/Misc_Tables/T_lights_4k_m3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Algorithms}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Decision\\  Epochs\end{tabular}}} & \multicolumn{4}{c|}{\textbf{Average Congestion}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Overall\\ Congestion\end{tabular}}} \\ \cline{3-6}
 &  & \textbf{$T_1$} & \textbf{$T_2$} & \textbf{$T_3$} & \textbf{$T_4$} &  \\ \hline \hline
\multirow{9}{*}{\textbf{MAAC}} & \textbf{1300} & 2.62199 & 3.13333 & 1.71068 & 2.60282 & 10.06882 \\ \cline{2-7} 
 & \textbf{1325} & 2.62274 & 3.13156 & 1.71052 & 2.60501 & 10.06983 \\ \cline{2-7} 
 & \textbf{1350} & 2.62485 & 3.13056 & 1.7106 & 2.60602 & 10.07203 \\ \cline{2-7} 
 & \textbf{1375} & 2.6294 & 3.13075 & 1.71187 & 2.60627 & 10.07829 \\ \cline{2-7} 
 & \textbf{1400} & 2.62791 & 3.13123 & 1.71119 & 2.60446 & 10.0748 \\ \cline{2-7} 
 & \textbf{1425} & 2.62784 & 3.12807 & 1.71212 & 2.60514 & 10.07318 \\ \cline{2-7} 
 & \textbf{1450} & 2.63029 & 3.12837 & 1.7141 & 2.60411 & 10.07688 \\ \cline{2-7} 
 & \textbf{1475} & 2.62617 & 3.12955 & 1.71366 & 2.60186 & 10.07124 \\ \cline{2-7} 
 & \textbf{1500} & 2.62749 & 3.12917 & 1.71324 & 2.60063 & 10.07052 \\ \hline \hline
\multirow{9}{*}{\textbf{FI-MAN}} & \textbf{1300} & 1.83053 & 2.67577 & 1.88261 & 1.98827 & 8.37719 \\ \cline{2-7} 
 & \textbf{1325} & 1.82942 & 2.67294 & 1.88228 & 1.9851 & 8.36975 \\ \cline{2-7} 
 & \textbf{1350} & 1.82712 & 2.6711 & 1.88621 & 1.98317 & 8.36759 \\ \cline{2-7} 
 & \textbf{1375} & 1.82426 & 2.66789 & 1.88955 & 1.9813 & 8.363 \\ \cline{2-7} 
 & \textbf{1400} & 1.82253 & 2.66732 & 1.88967 & 1.97816 & 8.35768 \\ \cline{2-7} 
 & \textbf{1425} & 1.82236 & 2.66418 & 1.89317 & 1.97707 & 8.35678 \\ \cline{2-7} 
 & \textbf{1450} & 1.82207 & 2.66251 & 1.89531 & 1.97369 & 8.35359 \\ \cline{2-7} 
 & \textbf{1475} & 1.81745 & 2.66389 & 1.89516 & 1.96922 & 8.34572 \\ \cline{2-7} 
 & \textbf{1500} & 1.81452 & 2.66271 & 1.89403 & 1.96866 & 8.33993 \\ \hline \hline
\multirow{9}{*}{\textbf{AP-MAN}} & \textbf{1300} & 2.62579 & 3.13521 & 1.7088 & 2.60818 & 10.07798 \\ \cline{2-7} 
 & \textbf{1325} & 2.6263 & 3.13396 & 1.70858 & 2.61047 & 10.07931 \\ \cline{2-7} 
 & \textbf{1350} & 2.6283 & 3.13372 & 1.70846 & 2.61133 & 10.0818 \\ \cline{2-7} 
 & \textbf{1375} & 2.63418 & 3.13362 & 1.70946 & 2.61241 & 10.08968 \\ \cline{2-7} 
 & \textbf{1400} & 2.63322 & 3.1347 & 1.70855 & 2.61039 & 10.08686 \\ \cline{2-7} 
 & \textbf{1425} & 2.63312 & 3.13182 & 1.70937 & 2.61096 & 10.08527 \\ \cline{2-7} 
 & \textbf{1450} & 2.63569 & 3.13216 & 1.7117 & 2.61062 & 10.09017 \\ \cline{2-7} 
 & \textbf{1475} & 2.63087 & 3.13382 & 1.71136 & 2.6087 & 10.08475 \\ \cline{2-7} 
 & \textbf{1500} & 2.63271 & 3.13333 & 1.71092 & 2.60794 & 10.08489 \\ \hline \hline
\multirow{9}{*}{\textbf{FIAP-MAN}} & \textbf{1300} & 1.94389 & 2.86851 & 1.64148 & 2.13928 & 8.59316 \\ \cline{2-7} 
 & \textbf{1325} & 1.93895 & 2.86478 & 1.64129 & 2.13613 & 8.58116 \\ \cline{2-7} 
 & \textbf{1350} & 1.93435 & 2.85891 & 1.64033 & 2.13182 & 8.5654 \\ \cline{2-7} 
 & \textbf{1375} & 1.93032 & 2.85503 & 1.64277 & 2.12751 & 8.55562 \\ \cline{2-7} 
 & \textbf{1400} & 1.92632 & 2.85212 & 1.64199 & 2.12346 & 8.54389 \\ \cline{2-7} 
 & \textbf{1425} & 1.92351 & 2.84679 & 1.64374 & 2.12173 & 8.53577 \\ \cline{2-7} 
 & \textbf{1450} & 1.92249 & 2.8436 & 1.64366 & 2.11664 & 8.52638 \\ \cline{2-7} 
 & \textbf{1475} & 1.91659 & 2.83846 & 1.64235 & 2.11282 & 8.51022 \\ \cline{2-7} 
 & \textbf{1500} & 1.91186 & 2.836 & 1.64116 & 2.11131 & 8.50033 \\ \hline
\end{tabular}
\caption{Avg congestion for all traffic lights.  $N_v = 40000$, mode 3.}
\end{table}

==> Tables-Traffic Light/Misc_Tables/T_lights_5k_m1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Algorithms}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Decision\\ Epochs\end{tabular}}} & \multicolumn{4}{c|}{\textbf{Average Congestion}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Overall \\ Congestion\end{tabular}}} \\ \cline{3-6}
 &  & $T_1$ & $T_2$ & $T_3$ & $T_4$ &  \\ \hline \hline
\multirow{5}{*}{\textbf{MAAC}} & \textbf{1300} & 3.48613 & 3.37825 & 3.34808 & 3.44544 & 13.6579 \\ \cline{2-7} 
% & \textbf{1325} & 3.48868 & 3.37755 & 3.35782 & 3.45412 & 13.67816 \\ \cline{2-7} 
 & \textbf{1350} & 3.48535 & 3.37478 & 3.36124 & 3.44845 & 13.66981 \\ \cline{2-7} 
%  & \textbf{1375} & 3.48205 & 3.37599 & 3.35683 & 3.44569 & 13.66056 \\ \cline{2-7} 
 & \textbf{1400} & 3.48167 & 3.37264 & 3.35452 & 3.44766 & 13.65649 \\ \cline{2-7} 
%  & \textbf{1425} & 3.48498 & 3.38062 & 3.35408 & 3.44301 & 13.66268 \\ \cline{2-7} 
 & \textbf{1450} & 3.48895 & 3.3812 & 3.34986 & 3.44187 & 13.66189 \\ \cline{2-7} 
%  & \textbf{1475} & 3.48305 & 3.38074 & 3.34703 & 3.43735 & 13.64818 \\ \cline{2-7} 
 & \textbf{1500} & 3.48135 & 3.3789 & 3.34787 & 3.4376 & 13.64571 \\ \hline \hline
\multirow{5}{*}{\textbf{FI-MAN}} & \textbf{1300} & 2.56024 & 2.55406 & 2.54095 & 2.60867 & 10.26393 \\ \cline{2-7} 
%  & \textbf{1325} & 2.55656 & 2.55053 & 2.53957 & 2.60986 & 10.25652 \\ \cline{2-7} 
 & \textbf{1350} & 2.55422 & 2.54652 & 2.53886 & 2.60486 & 10.24446 \\ \cline{2-7} 
%  & \textbf{1375} & 2.5505 & 2.54269 & 2.53577 & 2.60203 & 10.231 \\ \cline{2-7} 
 & \textbf{1400} & 2.5449 & 2.53971 & 2.53361 & 2.5987 & 10.21692 \\ \cline{2-7} 
%  & \textbf{1425} & 2.54274 & 2.53709 & 2.52886 & 2.59474 & 10.20342 \\ \cline{2-7} 
 & \textbf{1450} & 2.54099 & 2.53475 & 2.52435 & 2.59346 & 10.19354 \\ \cline{2-7} 
%  & \textbf{1475} & 2.53515 & 2.53183 & 2.51817 & 2.58811 & 10.17327 \\ \cline{2-7} 
 & \textbf{1500} & 2.53231 & 2.52956 & 2.51875 & 2.58925 & 10.16988 \\ \hline \hline
\multirow{5}{*}{\textbf{AP-MAN}} & \textbf{1300} & 3.51468 & 3.39959 & 3.37735 & 3.48793 & 13.77954 \\ \cline{2-7} 
%  & \textbf{1325} & 3.51553 & 3.40125 & 3.3857 & 3.49529 & 13.79778 \\ \cline{2-7} 
 & \textbf{1350} & 3.51448 & 3.39834 & 3.38832 & 3.49046 & 13.7916 \\ \cline{2-7} 
%  & \textbf{1375} & 3.5132 & 3.3989 & 3.38415 & 3.48771 & 13.78396 \\ \cline{2-7} 
 & \textbf{1400} & 3.51273 & 3.39686 & 3.38276 & 3.49027 & 13.78262 \\ \cline{2-7} 
%  & \textbf{1425} & 3.51491 & 3.40547 & 3.38185 & 3.48631 & 13.78853 \\ \cline{2-7} 
 & \textbf{1450} & 3.51785 & 3.40663 & 3.37742 & 3.4878 & 13.78971 \\ \cline{2-7} 
%  & \textbf{1475} & 3.51203 & 3.4059 & 3.37501 & 3.4834 & 13.77633 \\ \cline{2-7} 
 & \textbf{1500} & 3.51088 & 3.40409 & 3.37603 & 3.48474 & 13.77573 \\ \hline \hline
\multirow{5}{*}{\textbf{FIAP-MAN}} & \textbf{1300} & 2.59067 & 2.55827 & 2.56973 & 2.57903 & 10.29771 \\ \cline{2-7} 
%  & \textbf{1325} & 2.58799 & 2.55453 & 2.56676 & 2.58117 & 10.29044 \\ \cline{2-7} 
 & \textbf{1350} & 2.58557 & 2.54906 & 2.56444 & 2.57567 & 10.27473 \\ \cline{2-7} 
%  & \textbf{1375} & 2.58226 & 2.54595 & 2.56108 & 2.57263 & 10.26192 \\ \cline{2-7} 
 & \textbf{1400} & 2.57705 & 2.54379 & 2.55733 & 2.56851 & 10.24668 \\ \cline{2-7} 
%  & \textbf{1425} & 2.57574 & 2.54176 & 2.55373 & 2.5642 & 10.23542 \\ \cline{2-7} 
 & \textbf{1450} & 2.57375 & 2.54031 & 2.54917 & 2.5623 & 10.22554 \\ \cline{2-7} 
%  & \textbf{1475} & 2.56788 & 2.53694 & 2.54348 & 2.55643 & 10.20473 \\ \cline{2-7} 
 & \textbf{1500} & 2.5661 & 2.53445 & 2.54253 & 2.5555 & 10.19858 \\ \hline
\end{tabular}
\caption{$N_v = 50000$, mode 1.}
\label{Table: 5k_mode_1}
\end{table}

==> Tables-Traffic Light/Misc_Tables/T_lights_5k_m3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Algorithms}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Decision\\  Epochs\end{tabular}}} & \multicolumn{4}{c|}{\textbf{Average Congestion}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Overall\\ Congestion\end{tabular}}} \\ \cline{3-6}
 &  & \textbf{$T_1$} & \textbf{$T_2$} & \textbf{$T_3$} & \textbf{$T_4$} &  \\ \hline \hline
\multirow{9}{*}{\textbf{MAAC}} & \textbf{1300} & 3.74204 & 4.34403 & 2.24059 & 3.71553 & 14.04219 \\ \cline{2-7} 
 & \textbf{1325} & 3.74318 & 4.3465 & 2.24117 & 3.71894 & 14.04979 \\ \cline{2-7} 
 & \textbf{1350} & 3.73668 & 4.34487 & 2.23892 & 3.71686 & 14.03732 \\ \cline{2-7} 
 & \textbf{1375} & 3.7389 & 4.34453 & 2.24027 & 3.71255 & 14.03625 \\ \cline{2-7} 
 & \textbf{1400} & 3.74228 & 4.34359 & 2.2417 & 3.70765 & 14.03522 \\ \cline{2-7} 
 & \textbf{1425} & 3.74076 & 4.34576 & 2.24352 & 3.70547 & 14.0355 \\ \cline{2-7} 
 & \textbf{1450} & 3.74119 & 4.34666 & 2.2463 & 3.70492 & 14.03906 \\ \cline{2-7} 
 & \textbf{1475} & 3.73178 & 4.33952 & 2.24721 & 3.70361 & 14.02212 \\ \cline{2-7} 
 & \textbf{1500} & 3.73327 & 4.33586 & 2.24885 & 3.69889 & 14.01687 \\ \hline \hline
\multirow{9}{*}{\textbf{FI-MAN}} & \textbf{1300} & 2.65176 & 4.51508 & 2.35887 & 2.59801 & 12.12372 \\ \cline{2-7} 
 & \textbf{1325} & 2.64542 & 4.51225 & 2.35831 & 2.59618 & 12.11215 \\ \cline{2-7} 
 & \textbf{1350} & 2.63825 & 4.51568 & 2.3576 & 2.58895 & 12.10048 \\ \cline{2-7} 
 & \textbf{1375} & 2.63589 & 4.51383 & 2.35863 & 2.58458 & 12.09293 \\ \cline{2-7} 
 & \textbf{1400} & 2.63344 & 4.51391 & 2.35818 & 2.57897 & 12.08449 \\ \cline{2-7} 
 & \textbf{1425} & 2.62902 & 4.51411 & 2.35985 & 2.57541 & 12.0784 \\ \cline{2-7} 
 & \textbf{1450} & 2.62329 & 4.51483 & 2.36137 & 2.56899 & 12.06849 \\ \cline{2-7} 
 & \textbf{1475} & 2.61729 & 4.50381 & 2.35852 & 2.56563 & 12.04525 \\ \cline{2-7} 
 & \textbf{1500} & 2.61303 & 4.49239 & 2.35911 & 2.56366 & 12.02819 \\ \hline \hline
\multirow{9}{*}{\textbf{AP-MAN}} & \textbf{1300} & 3.75367 & 4.34856 & 2.23625 & 3.7583 & 14.09678 \\ \cline{2-7} 
 & \textbf{1325} & 3.75373 & 4.3497 & 2.23708 & 3.76258 & 14.1031 \\ \cline{2-7} 
 & \textbf{1350} & 3.74742 & 4.34587 & 2.23461 & 3.76091 & 14.08882 \\ \cline{2-7} 
 & \textbf{1375} & 3.75226 & 4.34665 & 2.23626 & 3.7568 & 14.09196 \\ \cline{2-7} 
 & \textbf{1400} & 3.75537 & 4.34535 & 2.23848 & 3.75136 & 14.09055 \\ \cline{2-7} 
 & \textbf{1425} & 3.75282 & 4.34809 & 2.2397 & 3.75026 & 14.09087 \\ \cline{2-7} 
 & \textbf{1450} & 3.75636 & 4.34781 & 2.24272 & 3.75213 & 14.09902 \\ \cline{2-7} 
 & \textbf{1475} & 3.74684 & 4.34028 & 2.24399 & 3.7511 & 14.08221 \\ \cline{2-7} 
 & \textbf{1500} & 3.74765 & 4.33786 & 2.24715 & 3.74634 & 14.07899 \\ \hline \hline
\multirow{9}{*}{\textbf{FIAP-MAN}} & \textbf{1300} & 2.75657 & 3.85462 & 1.9291 & 2.93889 & 11.47918 \\ \cline{2-7} 
 & \textbf{1325} & 2.74987 & 3.8458 & 1.92624 & 2.93507 & 11.45698 \\ \cline{2-7} 
 & \textbf{1350} & 2.74275 & 3.83252 & 1.92256 & 2.92593 & 11.42376 \\ \cline{2-7} 
 & \textbf{1375} & 2.737 & 3.82576 & 1.91898 & 2.91857 & 11.40031 \\ \cline{2-7} 
 & \textbf{1400} & 2.73475 & 3.82733 & 1.91597 & 2.9104 & 11.38845 \\ \cline{2-7} 
 & \textbf{1425} & 2.72937 & 3.82087 & 1.91335 & 2.90546 & 11.36905 \\ \cline{2-7} 
 & \textbf{1450} & 2.72273 & 3.80949 & 1.91254 & 2.89702 & 11.34178 \\ \cline{2-7} 
 & \textbf{1475} & 2.71512 & 3.79772 & 1.91044 & 2.88878 & 11.31207 \\ \cline{2-7} 
 & \textbf{1500} & 2.71129 & 3.78486 & 1.90733 & 2.88309 & 11.28657 \\ \hline
\end{tabular}
\caption{$N_v = 50000$ mode 3.}
\end{table}

==> Tables-Traffic Light/Misc_Tables/Table_mode1_40000.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Algorithms} & \textbf{\begin{tabular}[c]{@{}c@{}}Decision\\ Epoch\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Average\\ Congestion\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Standard\\ Deviation\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Confidence\\ Interval (95\%)\end{tabular}} \\ \hline \hline
\multirow{9}{*}{\textbf{MAAC}} & \textbf{1300} & 10.07062 & 0.10894 & (10.00310, 10.13814) \\ \cline{2-5} 
 & \textbf{1325} & 10.07405 & 0.10759 & (10.00737, 10.14073) \\ \cline{2-5} 
 & \textbf{1350} & 10.06115 & 0.11062 & (9.99259, 10.12971) \\ \cline{2-5} 
 & \textbf{1375} & 10.05710 & 0.10893 & (9.98959, 10.12461) \\ \cline{2-5} 
 & \textbf{1400} & 10.05850 & 0.10435 & (9.99382, 10.12318) \\ \cline{2-5} 
 & \textbf{1425} & 10.05437 & 0.10619 & (9.98855, 10.12019) \\ \cline{2-5} 
 & \textbf{1450} & 10.05539 & 0.10314 & (9.99146, 10.11932) \\ \cline{2-5} 
 & \textbf{1475} & 10.04889 & 0.10604 & (9.98317, 10.11461) \\ \cline{2-5} 
 & \textbf{1500} & 10.05136 & 0.09941 & (9.98975, 10.11297) \\ \hline \hline
\multirow{9}{*}{\textbf{FI-MAN}} & \textbf{1300} & 8.17687 & 0.79232 & (7.68579, 8.66795) \\ \cline{2-5} 
 & \textbf{1325} & 8.16979 & 0.78395 & (7.68390, 8.65568) \\ \cline{2-5} 
 & \textbf{1350} & 8.15568 & 0.77169 & (7.67739, 8.63397) \\ \cline{2-5} 
 & \textbf{1375} & 8.14285 & 0.75892 & (7.67248, 8.61322) \\ \cline{2-5} 
 & \textbf{1400} & 8.13102 & 0.74244 & (7.67086, 8.59118) \\ \cline{2-5} 
 & \textbf{1425} & 8.11878 & 0.73214 & (7.66500, 8.57256) \\ \cline{2-5} 
 & \textbf{1450} & 8.10304 & 0.72265 & (7.65515, 8.55093) \\ \cline{2-5} 
 & \textbf{1475} & 8.08962 & 0.71614 & (7.64576, 8.53348) \\ \cline{2-5} 
 & \textbf{1500} & 8.07926 & 0.71115 & (7.63849, 8.52003) \\ \hline \hline
\multirow{9}{*}{\textbf{AP-MAN}} & \textbf{1300} & 10.08229 & 0.11097 & (10.01351, 10.15107) \\ \cline{2-5} 
 & \textbf{1325} & 10.08569 & 0.10746 & (10.01909, 10.15229) \\ \cline{2-5} 
 & \textbf{1350} & 10.07259 & 0.11124 & (10.00364, 10.14154) \\ \cline{2-5} 
 & \textbf{1375} & 10.06829 & 0.10814 & (10.00127, 10.13531) \\ \cline{2-5} 
 & \textbf{1400} & 10.07052 & 0.10252 & (10.00698, 10.13406) \\ \cline{2-5} 
 & \textbf{1425} & 10.06620 & 0.10445 & (10.00146, 10.13094) \\ \cline{2-5} 
 & \textbf{1450} & 10.06713 & 0.09998 & (10.00516, 10.12910) \\ \cline{2-5} 
 & \textbf{1475} & 10.06165 & 0.10334 & (9.99760, 10.12570) \\ \cline{2-5} 
 & \textbf{1500} & 10.06477 & 0.09796 & (10.00405, 10.12549) \\ \hline \hline
\multirow{9}{*}{\textbf{FIAP-MAN}} & \textbf{1300} & 7.82611 & 0.13524 & (7.74229, 7.90993) \\ \cline{2-5} 
 & \textbf{1325} & 7.82406 & 0.13537 & (7.74016, 7.90796) \\ \cline{2-5} 
 & \textbf{1350} & 7.81535 & 0.13211 & (7.73347, 7.89723) \\ \cline{2-5} 
 & \textbf{1375} & 7.80973 & 0.12820 & (7.73027, 7.88919) \\ \cline{2-5} 
 & \textbf{1400} & 7.80447 & 0.12500 & (7.72700, 7.88194) \\ \cline{2-5} 
 & \textbf{1425} & 7.79581 & 0.11999 & (7.72144, 7.87018) \\ \cline{2-5} 
 & \textbf{1450} & 7.78483 & 0.11916 & (7.71098, 7.85868) \\ \cline{2-5} 
 & \textbf{1475} & 7.77594 & 0.11951 & (7.70187, 7.85001) \\ \cline{2-5} 
 & \textbf{1500} & 7.77147 & 0.11883 & (7.69782, 7.84512) \\ \hline
\end{tabular}
\caption{Arrival pattern 1. $N_v = 40000$.}
\end{table}

==> Tables-Traffic Light/Misc_Tables/Table_mode1_50000.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Algorithms} & \textbf{\begin{tabular}[c]{@{}c@{}}Decision\\  Epochs\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Average \\ Congestion\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Standard \\ Deviation\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Confidence \\ Interval (95\%)\end{tabular}} \\ \hline \hline
\multirow{9}{*}{\textbf{MAAC}} & \textbf{1300} & 13.65790 & 0.20956 & (13.52802, 13.78778) \\ \cline{2-5} 
 & \textbf{1325} & 13.67816 & 0.20409 & (13.55167, 13.80465) \\ \cline{2-5} 
 & \textbf{1350} & 13.66981 & 0.21010 & (13.53959, 13.80003) \\ \cline{2-5} 
 & \textbf{1375} & 13.66056 & 0.20991 & (13.53046, 13.79066) \\ \cline{2-5} 
 & \textbf{1400} & 13.65649 & 0.20735 & (13.52798, 13.78500) \\ \cline{2-5} 
 & \textbf{1425} & 13.66268 & 0.19949 & (13.53904, 13.78632) \\ \cline{2-5} 
 & \textbf{1450} & 13.66189 & 0.21023 & (13.53159, 13.79219) \\ \cline{2-5} 
 & \textbf{1475} & 13.64818 & 0.20464 & (13.52135, 13.77501) \\ \cline{2-5} 
 & \textbf{1500} & 13.64571 & 0.19755 & (13.52327, 13.76815) \\ \hline \hline
\multirow{9}{*}{\textbf{FI-MAN}} & \textbf{1300} & 10.26393 & 0.13996 & (10.17718, 10.35068) \\ \cline{2-5} 
 & \textbf{1325} & 10.25652 & 0.13113 & (10.17525, 10.33779) \\ \cline{2-5} 
 & \textbf{1350} & 10.24446 & 0.13366 & (10.16162, 10.32730) \\ \cline{2-5} 
 & \textbf{1375} & 10.23100 & 0.13073 & (10.14997, 10.31203) \\ \cline{2-5} 
 & \textbf{1400} & 10.21692 & 0.12768 & (10.13778, 10.29606) \\ \cline{2-5} 
 & \textbf{1425} & 10.20342 & 0.12244 & (10.12753, 10.27931) \\ \cline{2-5} 
 & \textbf{1450} & 10.19354 & 0.11760 & (10.12065, 10.26643) \\ \cline{2-5} 
 & \textbf{1475} & 10.17327 & 0.11501 & (10.10199, 10.24455) \\ \cline{2-5} 
 & \textbf{1500} & 10.16988 & 0.11877 & (10.09627, 10.24349) \\ \hline \hline
\multirow{9}{*}{\textbf{AP-MAN}} & \textbf{1300} & 13.77954 & 0.20823 & (13.65048, 13.90860) \\ \cline{2-5} 
 & \textbf{1325} & 13.79778 & 0.20028 & (13.67365, 13.92191) \\ \cline{2-5} 
 & \textbf{1350} & 13.79160 & 0.20285 & (13.66587, 13.91733) \\ \cline{2-5} 
 & \textbf{1375} & 13.78396 & 0.19820 & (13.66112, 13.90680) \\ \cline{2-5} 
 & \textbf{1400} & 13.78262 & 0.19888 & (13.65936, 13.90588) \\ \cline{2-5} 
 & \textbf{1425} & 13.78853 & 0.18912 & (13.67131, 13.90575) \\ \cline{2-5} 
 & \textbf{1450} & 13.78971 & 0.20300 & (13.66389, 13.91553) \\ \cline{2-5} 
 & \textbf{1475} & 13.77633 & 0.19721 & (13.65410, 13.89856) \\ \cline{2-5} 
 & \textbf{1500} & 13.77573 & 0.18925 & (13.65843, 13.89303) \\ \hline \hline
\multirow{9}{*}{\textbf{FIAP-MAN}} & \textbf{1300} & 10.29771 & 0.22585 & (10.15773, 10.43769) \\ \cline{2-5} 
 & \textbf{1325} & 10.29044 & 0.22041 & (10.15383, 10.42705) \\ \cline{2-5} 
 & \textbf{1350} & 10.27473 & 0.21690 & (10.14030, 10.40916) \\ \cline{2-5} 
 & \textbf{1375} & 10.26192 & 0.21626 & (10.12788, 10.39596) \\ \cline{2-5} 
 & \textbf{1400} & 10.24668 & 0.21714 & (10.11210, 10.38126) \\ \cline{2-5} 
 & \textbf{1425} & 10.23542 & 0.20928 & (10.10571, 10.36513) \\ \cline{2-5} 
 & \textbf{1450} & 10.22554 & 0.20637 & (10.09763, 10.35345) \\ \cline{2-5} 
 & \textbf{1475} & 10.20473 & 0.20924 & (10.07504, 10.33442) \\ \cline{2-5} 
 & \textbf{1500} & 10.19858 & 0.21248 & (10.06689, 10.33027) \\ \hline
\end{tabular}
\caption{The average congestion, standard deviation, and 95\% confidence interval of algorithms when the vehicle is assigned to a source node according to  the probability vector corresponding to arrival pattern 1. These values are obtained by averaging over ten runs. $N_v = 50000 $, mode 1} 
\label{table: mode1_50000}
\end{table}

==> Tables-Traffic Light/Misc_Tables/Table_mode2_40000.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Algorithms} & \textbf{\begin{tabular}[c]{@{}c@{}}Decision\\ Epoch\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Average\\ Congestion\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Standard\\ Deviation\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Confidence\\ Interval (95\%)\end{tabular}} \\ \hline \hline
\multirow{9}{*}{\textbf{MAAC}} & \textbf{1300} & 10.12001 & 0.11923 & (10.04611, 10.19391) \\ \cline{2-5} 
 & \textbf{1325} & 10.12350 & 0.10930 & (10.05576, 10.19124) \\ \cline{2-5} 
 & \textbf{1350} & 10.12436 & 0.10631 & (10.05847, 10.19025) \\ \cline{2-5} 
 & \textbf{1375} & 10.12537 & 0.11112 & (10.05650, 10.19424) \\ \cline{2-5} 
 & \textbf{1400} & 10.12559 & 0.10506 & (10.06047, 10.19071) \\ \cline{2-5} 
 & \textbf{1425} & 10.12375 & 0.10735 & (10.05722, 10.19028) \\ \cline{2-5} 
 & \textbf{1450} & 10.12758 & 0.10464 & (10.06272, 10.19244) \\ \cline{2-5} 
 & \textbf{1475} & 10.12046 & 0.10211 & (10.05717, 10.18375) \\ \cline{2-5} 
 & \textbf{1500} & 10.11135 & 0.10140 & (10.04850, 10.17420) \\ \hline \hline
\multirow{9}{*}{\textbf{FI-MAN}} & \textbf{1300} & 8.11726 & 0.64136 & (7.71975, 8.51477) \\ \cline{2-5} 
 & \textbf{1325} & 8.11195 & 0.64113 & (7.71458, 8.50932) \\ \cline{2-5} 
 & \textbf{1350} & 8.10156 & 0.65350 & (7.69652, 8.50660) \\ \cline{2-5} 
 & \textbf{1375} & 8.09285 & 0.66326 & (7.68176, 8.50394) \\ \cline{2-5} 
 & \textbf{1400} & 8.08654 & 0.66579 & (7.67389, 8.49919) \\ \cline{2-5} 
 & \textbf{1425} & 8.07789 & 0.66711 & (7.66442, 8.49136) \\ \cline{2-5} 
 & \textbf{1450} & 8.06486 & 0.66347 & (7.65364, 8.47608) \\ \cline{2-5} 
 & \textbf{1475} & 8.05206 & 0.65900 & (7.64362, 8.46050) \\ \cline{2-5} 
 & \textbf{1500} & 8.04344 & 0.65241 & (7.63908, 8.44780) \\ \hline \hline
\multirow{9}{*}{\textbf{AP-MAN}} & \textbf{1300} & 10.13065 & 0.11139 & (10.06161, 10.19969) \\ \cline{2-5} 
 & \textbf{1325} & 10.13358 & 0.10212 & (10.07029, 10.19687) \\ \cline{2-5} 
 & \textbf{1350} & 10.13363 & 0.09800 & (10.07289, 10.19437) \\ \cline{2-5} 
 & \textbf{1375} & 10.13474 & 0.10254 & (10.07119, 10.19829) \\ \cline{2-5} 
 & \textbf{1400} & 10.13549 & 0.09825 & (10.07460, 10.19638) \\ \cline{2-5} 
 & \textbf{1425} & 10.13295 & 0.10003 & (10.07095, 10.19495) \\ \cline{2-5} 
 & \textbf{1450} & 10.13565 & 0.09842 & (10.07465, 10.19665) \\ \cline{2-5} 
 & \textbf{1475} & 10.12870 & 0.09516 & (10.06972, 10.18768) \\ \cline{2-5} 
 & \textbf{1500} & 10.12087 & 0.09451 & (10.06229, 10.17945) \\ \hline \hline
\multirow{9}{*}{\textbf{FIAP-MAN}} & \textbf{1300} & 7.78031 & 0.13720 & (7.69527, 7.86535) \\ \cline{2-5} 
 & \textbf{1325} & 7.77637 & 0.13122 & (7.69504, 7.85770) \\ \cline{2-5} 
 & \textbf{1350} & 7.76481 & 0.13353 & (7.68205, 7.84757) \\ \cline{2-5} 
 & \textbf{1375} & 7.75480 & 0.13985 & (7.66812, 7.84148) \\ \cline{2-5} 
 & \textbf{1400} & 7.74760 & 0.13177 & (7.66593, 7.82927) \\ \cline{2-5} 
 & \textbf{1425} & 7.73925 & 0.13471 & (7.65576, 7.82274) \\ \cline{2-5} 
 & \textbf{1450} & 7.73017 & 0.13674 & (7.64542, 7.81492) \\ \cline{2-5} 
 & \textbf{1475} & 7.71843 & 0.13188 & (7.63669, 7.80017) \\ \cline{2-5} 
 & \textbf{1500} & 7.71313 & 0.12894 & (7.63321, 7.79305) \\ \hline
\end{tabular}
\caption{Arrival pattern $1^{\prime}$. $N_v = 40000$}
\end{table}

==> Tables-Traffic Light/Misc_Tables/Table_mode2_50000.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Algorithms} & \textbf{\begin{tabular}[c]{@{}c@{}}Decision\\  Epochs\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Average \\ Congestion\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Standard \\ Deviation\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Confidence \\ Interval (95\%)\end{tabular}} \\ \hline \hline
\multirow{9}{*}{\textbf{MAAC}} & \textbf{1300} & 14.17963 & 0.15649 & (14.08264, 14.27662) \\ \cline{2-5} 
 & \textbf{1325} & 14.18470 & 0.15039 & (14.09149, 14.27791) \\ \cline{2-5} 
 & \textbf{1350} & 14.17159 & 0.13754 & (14.08634, 14.25684) \\ \cline{2-5} 
 & \textbf{1375} & 14.17948 & 0.11981 & (14.10522, 14.25374) \\ \cline{2-5} 
 & \textbf{1400} & 14.19757 & 0.10640 & (14.13162, 14.26352) \\ \cline{2-5} 
 & \textbf{1425} & 14.20464 & 0.11549 & (14.13306, 14.27622) \\ \cline{2-5} 
 & \textbf{1450} & 14.21093 & 0.11033 & (14.14255, 14.27931) \\ \cline{2-5} 
 & \textbf{1475} & 14.20000 & 0.11257 & (14.13023, 14.26977) \\ \cline{2-5} 
 & \textbf{1500} & 14.20165 & 0.10245 & (14.13815, 14.26515) \\ \hline \hline
\multirow{9}{*}{\textbf{FI-MAN}} & \textbf{1300} & 10.34792 & 0.15244 & (10.25344, 10.44240) \\ \cline{2-5} 
 & \textbf{1325} & 10.33968 & 0.15526 & (10.24345, 10.43591) \\ \cline{2-5} 
 & \textbf{1350} & 10.32218 & 0.15505 & (10.22608, 10.41828) \\ \cline{2-5} 
 & \textbf{1375} & 10.31042 & 0.14989 & (10.21752, 10.40332) \\ \cline{2-5} 
 & \textbf{1400} & 10.30118 & 0.14983 & (10.20832, 10.39404) \\ \cline{2-5} 
 & \textbf{1425} & 10.29229 & 0.14524 & (10.20227, 10.38231) \\ \cline{2-5} 
 & \textbf{1450} & 10.27953 & 0.14173 & (10.19169, 10.36737) \\ \cline{2-5} 
 & \textbf{1475} & 10.26077 & 0.14192 & (10.17281, 10.34873) \\ \cline{2-5} 
 & \textbf{1500} & 10.25633 & 0.14000 & (10.16956, 10.34310) \\ \hline \hline
\multirow{9}{*}{\textbf{AP-MAN}} & \textbf{1300} & 14.22500 & 0.17367 & (14.11736, 14.33264) \\ \cline{2-5} 
 & \textbf{1325} & 14.23449 & 0.16484 & (14.13232, 14.33666) \\ \cline{2-5} 
 & \textbf{1350} & 14.22331 & 0.15367 & (14.12807, 14.31855) \\ \cline{2-5} 
 & \textbf{1375} & 14.22753 & 0.13844 & (14.14173, 14.31333) \\ \cline{2-5} 
 & \textbf{1400} & 14.24721 & 0.12805 & (14.16785, 14.32657) \\ \cline{2-5} 
 & \textbf{1425} & 14.25385 & 0.13285 & (14.17151, 14.33619) \\ \cline{2-5} 
 & \textbf{1450} & 14.26026 & 0.12776 & (14.18107, 14.33945) \\ \cline{2-5} 
 & \textbf{1475} & 14.24961 & 0.13023 & (14.16889, 14.33033) \\ \cline{2-5} 
 & \textbf{1500} & 14.25049 & 0.12013 & (14.17603, 14.32495) \\ \hline \hline
\multirow{9}{*}{\textbf{FIAP-MAN}} & \textbf{1300} & 10.34760 & 0.20936 & (10.21784, 10.47736) \\ \cline{2-5} 
 & \textbf{1325} & 10.33750 & 0.21543 & (10.20398, 10.47102) \\ \cline{2-5} 
 & \textbf{1350} & 10.31540 & 0.21398 & (10.18278, 10.44802) \\ \cline{2-5} 
 & \textbf{1375} & 10.30083 & 0.20445 & (10.17411, 10.42755) \\ \cline{2-5} 
 & \textbf{1400} & 10.29388 & 0.21186 & (10.16257, 10.42519) \\ \cline{2-5} 
 & \textbf{1425} & 10.28777 & 0.20968 & (10.15781, 10.41773) \\ \cline{2-5} 
 & \textbf{1450} & 10.27313 & 0.20298 & (10.14732, 10.39894) \\ \cline{2-5} 
 & \textbf{1475} & 10.25506 & 0.19558 & (10.13384, 10.37628) \\ \cline{2-5} 
 & \textbf{1500} & 10.24845 & 0.19404 & (10.12818, 10.36872) \\ \hline
\end{tabular}
\caption{The average congestion, standard deviation, and 95\% confidence interval of algorithms when the vehicle is assigned to a source node according to  the probability vector corresponding to arrival pattern 2. These values are obtained by averaging over ten runs. $N_v = 50000$, mode 2} 
\label{table: mode2_50000}
\end{table}

==> Tables-Traffic Light/Mode 1/Each_light_50K.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{lscape}
% \begin{landscape}
\begin{table}[h!]
\centering
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Algorithms}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Decision\\ Epoch\end{tabular}}} & \multicolumn{2}{c|}{\textbf{$T_1$ Congestion}} & \multicolumn{2}{c|}{\textbf{$T_2$ Congestion}} & \multicolumn{2}{c|}{\textbf{$T_3$ Congestion}} & \multicolumn{2}{c|}{\textbf{$T_4$ Congestion}} & \multicolumn{3}{c|}{\textbf{Network Congestion}} \\ \cline{3-13} 
 &  & \textbf{Average} & \textbf{CF} & \textbf{Average} & \textbf{CF} & \textbf{Average} & \textbf{CF} & \textbf{Average} & \textbf{CF} & \textbf{Average} & \textbf{Std Dvn} & \textbf{CI (95\%)} \\ \hline \hline
\multirow{5}{*}{\textbf{MAAC}} & 1300 & 3.74204 & 0.07054 & 4.34403 & 0.04921 & 2.24059 & 0.01216 & 3.71553 & 0.04491 & 14.04219 & 0.08587 & (13.98897, 14.09541) \\ \cline{2-13} 
 & 1350 & 3.73668 & 0.07196 & 4.34487 & 0.04956 & 2.23892 & 0.01078 & 3.71686 & 0.0413 & 14.03732 & 0.08768 & (13.98298, 14.09166) \\ \cline{2-13} 
 & 1400 & 3.74228 & 0.06496 & 4.34359 & 0.04945 & 2.2417 & 0.01108 & 3.70765 & 0.04154 & 14.03522 & 0.06993 & (13.99188, 14.07856) \\ \cline{2-13} 
 & 1450 & 3.74119 & 0.06109 & 4.34666 & 0.05252 & 2.2463 & 0.01084 & 3.70492 & 0.04242 & 14.03906 & 0.07464 & (13.9928, 14.08532) \\ \cline{2-13} 
 & 1500 & 3.73327 & 0.06693 & 4.33586 & 0.0502 & 2.24885 & 0.0129 & 3.69889 & 0.04 & 14.01687 & 0.08405 & (13.96478, 14.06896) \\ \hline \hline
\multirow{5}{*}{\textbf{FI-MAN}} & 1300 & 2.65176 & 0.11358 & 4.51508 & 0.83823 & 2.35887 & 0.15852 & 2.59801 & 0.04145 & 12.12372 & 1.44496 & (11.22814, 13.0193) \\ \cline{2-13} 
 & 1350 & 2.63825 & 0.11192 & 4.51568 & 0.85121 & 2.3576 & 0.15936 & 2.58895 & 0.04177 & 12.10048 & 1.45755 & (11.1971, 13.00386) \\ \cline{2-13} 
 & 1400 & 2.63344 & 0.11027 & 4.51391 & 0.85613 & 2.35818 & 0.1596 & 2.57897 & 0.03919 & 12.08449 & 1.46756 & (11.1749, 12.99408) \\ \cline{2-13} 
 & 1450 & 2.62329 & 0.11136 & 4.51483 & 0.87084 & 2.36137 & 0.16083 & 2.56899 & 0.03894 & 12.06849 & 1.48525 & (11.14794, 12.98904) \\ \cline{2-13} 
 & 1500 & 2.61303 & 0.11028 & 4.49239 & 0.86773 & 2.35911 & 0.16113 & 2.56366 & 0.0378 & 12.02819 & 1.48071 & (11.11045, 12.94593) \\ \hline \hline
\multirow{5}{*}{\textbf{AP-MAN}} & 1300 & 3.75367 & 0.07695 & 4.34856 & 0.04544 & 2.23625 & 0.01267 & 3.7583 & 0.04079 & 14.09678 & 0.07737 & (14.04883, 14.14473) \\ \cline{2-13} 
 & 1350 & 3.74742 & 0.07847 & 4.34587 & 0.04597 & 2.23461 & 0.01088 & 3.76091 & 0.03584 & 14.08882 & 0.07551 & (14.04202, 14.13562) \\ \cline{2-13} 
 & 1400 & 3.75537 & 0.07186 & 4.34535 & 0.04548 & 2.23848 & 0.01126 & 3.75136 & 0.03699 & 14.09055 & 0.06271 & (14.05168, 14.12942) \\ \cline{2-13} 
 & 1450 & 3.75636 & 0.06847 & 4.34781 & 0.04785 & 2.24272 & 0.01063 & 3.75213 & 0.04069 & 14.09902 & 0.06632 & (14.05792, 14.14012) \\ \cline{2-13} 
 & 1500 & 3.74765 & 0.07254 & 4.33786 & 0.04598 & 2.24715 & 0.01304 & 3.74634 & 0.03851 & 14.07899 & 0.08266 & (14.02776, 14.13022) \\ \hline \hline
\multirow{5}{*}{\textbf{FIAP-MAN}} & 1300 & 2.75657 & 0.24467 & 3.85462 & 0.37566 & 1.9291 & 0.14765 & 2.93889 & 0.16472 & 11.47918 & 1.11561 & (10.78773, 12.17063) \\ \cline{2-13} 
 & 1350 & 2.74275 & 0.23584 & 3.83252 & 0.37229 & 1.92256 & 0.14911 & 2.92593 & 0.16099 & 11.42376 & 1.09733 & (10.74364, 12.10388) \\ \cline{2-13} 
 & 1400 & 2.73475 & 0.22884 & 3.82733 & 0.38336 & 1.91597 & 0.147 & 2.9104 & 0.15614 & 11.38845 & 1.08963 & (10.7131, 12.0638) \\ \cline{2-13} 
 & 1450 & 2.72273 & 0.22165 & 3.80949 & 0.37969 & 1.91254 & 0.14879 & 2.89702 & 0.15159 & 11.34178 & 1.06876 & (10.67937, 12.00419) \\ \cline{2-13} 
 & 1500 & 2.71129 & 0.21358 & 3.78486 & 0.37062 & 1.90733 & 0.14817 & 2.88309 & 0.14706 & 11.28657 & 1.04137 & (10.64113, 11.93201) \\ \hline
\end{tabular}
\caption{50K Pattern 1. Each Light}
\label{table: 50K_each_light_pattern_1}
\end{table}
% \end{landscape}

==> Tables-Traffic Light/Mode 2/Each_light_50K.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{lscape}
\begin{landscape}
\begin{table}[h!]
\centering
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{|c|c|r|r|r|r|r|r|r|r|r|r|l|}
\hline
\multirow{2}{*}{\textbf{Algorithms}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Decision\\ Epoch\end{tabular}}} & \multicolumn{2}{c|}{\textbf{$T_1$ Congestion}} & \multicolumn{2}{c|}{\textbf{$T_1$ Congestion}} & \multicolumn{2}{c|}{\textbf{$T_3$ Congestion}} & \multicolumn{2}{c|}{\textbf{$T_4$ Congestion}} & \multicolumn{3}{c|}{\textbf{Network Congestion}} \\ \cline{3-13} 
 &  & \multicolumn{1}{c|}{\textbf{Average}} & \multicolumn{1}{c|}{\textbf{CF}} & \multicolumn{1}{c|}{\textbf{Average}} & \multicolumn{1}{c|}{\textbf{CF}} & \multicolumn{1}{c|}{\textbf{Average}} & \multicolumn{1}{c|}{\textbf{CF}} & \multicolumn{1}{c|}{\textbf{Average}} & \multicolumn{1}{c|}{\textbf{CF}} & \multicolumn{1}{c|}{\textbf{Average}} & \multicolumn{1}{c|}{\textbf{Std Dvn}} & \multicolumn{1}{c|}{\textbf{CI (95\%)}} \\ \hline
\multirow{5}{*}{\textbf{MAAC}} & 1300 & 3.48613 & 0.07369 & 3.37825 & 0.0314 & 3.34808 & 0.04214 & 3.44544 & 0.03706 & 13.6579 & 0.20956 & (13.52802, 13.78778) \\ \cline{2-13} 
 & 1350 & 3.48535 & 0.07283 & 3.37478 & 0.03094 & 3.36124 & 0.04133 & 3.44845 & 0.03451 & 13.66981 & 0.2101 & (13.53959, 13.80003) \\ \cline{2-13} 
 & 1400 & 3.48167 & 0.07123 & 3.37264 & 0.03411 & 3.35452 & 0.03959 & 3.44766 & 0.033 & 13.65649 & 0.20735 & (13.52798, 13.785) \\ \cline{2-13} 
 & 1450 & 3.48895 & 0.07275 & 3.3812 & 0.0347 & 3.34986 & 0.03445 & 3.44187 & 0.03648 & 13.66189 & 0.21023 & (13.53159, 13.79219) \\ \cline{2-13} 
 & 1500 & 3.48135 & 0.07022 & 3.3789 & 0.03437 & 3.34787 & 0.03225 & 3.4376 & 0.03317 & 13.64571 & 0.19755 & (13.52327, 13.76815) \\ \hline
\multirow{5}{*}{\textbf{FI-MAN}} & 1300 & 2.56024 & 0.0481 & 2.55406 & 0.04112 & 2.54095 & 0.04567 & 2.60867 & 0.0516 & 10.26393 & 0.13996 & (10.17718, 10.35068) \\ \cline{2-13} 
 & 1350 & 2.55422 & 0.047 & 2.54652 & 0.0442 & 2.53886 & 0.04525 & 2.60486 & 0.04825 & 10.24446 & 0.13366 & (10.16162, 10.3273) \\ \cline{2-13} 
 & 1400 & 2.5449 & 0.04746 & 2.53971 & 0.04345 & 2.53361 & 0.04357 & 2.5987 & 0.04685 & 10.21692 & 0.12768 & (10.13778, 10.29606) \\ \cline{2-13} 
 & 1450 & 2.54099 & 0.04608 & 2.53475 & 0.03961 & 2.52435 & 0.04443 & 2.59346 & 0.04546 & 10.19354 & 0.1176 & (10.12065, 10.26643) \\ \cline{2-13} 
 & 1500 & 2.53231 & 0.04671 & 2.52956 & 0.0403 & 2.51875 & 0.04505 & 2.58925 & 0.04524 & 10.16988 & 0.11877 & (10.09627, 10.24349) \\ \hline
\multirow{5}{*}{\textbf{AP-MAN}} & 1300 & 3.51468 & 0.07019 & 3.39959 & 0.02629 & 3.37735 & 0.04565 & 3.48793 & 0.03694 & 10.29771 & 0.22585 & (13.65048, 13.9086) \\ \cline{2-13} 
 & 1350 & 3.51448 & 0.06726 & 3.39834 & 0.02814 & 3.38832 & 0.04508 & 3.49046 & 0.03116 & 10.27473 & 0.2169 & (13.66587, 13.91733) \\ \cline{2-13} 
 & 1400 & 3.51273 & 0.06403 & 3.39686 & 0.03165 & 3.38276 & 0.04288 & 3.49027 & 0.02948 & 10.24668 & 0.21714 & (13.65936, 13.90588) \\ \cline{2-13} 
 & 1450 & 3.51785 & 0.06608 & 3.40663 & 0.0325 & 3.37742 & 0.03666 & 3.4878 & 0.0345 & 10.22554 & 0.20637 & (13.66389, 13.91553) \\ \cline{2-13} 
 & 1500 & 3.51088 & 0.06365 & 3.40409 & 0.03187 & 3.37603 & 0.03398 & 3.48474 & 0.03319 & 10.19858 & 0.21248 & (13.65843, 13.89303) \\ \hline
\multirow{5}{*}{\textbf{FIAP-MAN}} & 1300 & 2.59067 & 0.043 & 2.55827 & 0.03719 & 2.56973 & 0.04291 & 2.57903 & 0.03786 & \multicolumn{1}{c|}{11.47918} & \multicolumn{1}{c|}{1.11561} & (10.15773, 10.43769) \\ \cline{2-13} 
 & 1350 & 2.58557 & 0.04211 & 2.54906 & 0.03567 & 2.56444 & 0.04254 & 2.57567 & 0.03408 & \multicolumn{1}{c|}{11.42376} & \multicolumn{1}{c|}{1.09733} & (10.1403, 10.40916) \\ \cline{2-13} 
 & 1400 & 2.57705 & 0.04227 & 2.54379 & 0.03481 & 2.55733 & 0.04124 & 2.56851 & 0.03504 & \multicolumn{1}{c|}{11.38845} & \multicolumn{1}{c|}{1.08963} & (10.1121, 10.38126) \\ \cline{2-13} 
 & 1450 & 2.57375 & 0.03922 & 2.54031 & 0.03352 & 2.54917 & 0.0408 & 2.5623 & 0.03431 & \multicolumn{1}{c|}{11.34178} & \multicolumn{1}{c|}{1.06876} & (10.09763, 10.35345) \\ \cline{2-13} 
 & 1500 & 2.5661 & 0.04086 & 2.53445 & 0.03377 & 2.54253 & 0.04141 & 2.5555 & 0.03583 & \multicolumn{1}{c|}{11.28657} & \multicolumn{1}{c|}{1.04137} & (10.06689, 10.33027) \\ \hline
\end{tabular}
\caption{50K Pattern 2. Each Light}
\label{table: 50K_each_light_pattern_2}
\end{table}
\end{landscape}

==> Tables-Traffic Light/Mode 2prime/Each_light_50K.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{lscape}
\begin{landscape}
\begin{table}[h!]
\centering
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{|c|c|r|r|r|r|r|r|r|r|r|r|l|}
\hline
\multirow{2}{*}{\textbf{Algorithms}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Decision\\ Epoch\end{tabular}}} & \multicolumn{2}{c|}{\textbf{$T_1$ Congestion}} & \multicolumn{2}{c|}{\textbf{$T_1$ Congestion}} & \multicolumn{2}{c|}{\textbf{$T_3$ Congestion}} & \multicolumn{2}{c|}{\textbf{$T_4$ Congestion}} & \multicolumn{3}{c|}{\textbf{Network Congestion}} \\ \cline{3-13} 
 &  & \multicolumn{1}{c|}{\textbf{Average}} & \multicolumn{1}{c|}{\textbf{CF}} & \multicolumn{1}{c|}{\textbf{Average}} & \multicolumn{1}{c|}{\textbf{CF}} & \multicolumn{1}{c|}{\textbf{Average}} & \multicolumn{1}{c|}{\textbf{CF}} & \multicolumn{1}{c|}{\textbf{Average}} & \multicolumn{1}{c|}{\textbf{CF}} & \multicolumn{1}{c|}{\textbf{Average}} & \multicolumn{1}{c|}{\textbf{Std Dvn}} & \multicolumn{1}{c|}{\textbf{CI (95\%)}} \\ \hline
\multirow{5}{*}{\textbf{MAAC}} & 1300 & 3.43471 & 0.04688 & 3.65303 & 0.05684 & 3.65838 & 0.07218 & 3.4335 & 0.03213 & 14.17963 & 0.15649 & (14.08264, 14.27662) \\ \cline{2-13} 
 & 1350 & 3.43065 & 0.0448 & 3.64533 & 0.05281 & 3.6632 & 0.0634 & 3.43241 & 0.03483 & 14.17159 & 0.13754 & (14.08634, 14.25684) \\ \cline{2-13} 
 & 1400 & 3.44761 & 0.04453 & 3.65419 & 0.05393 & 3.65968 & 0.06263 & 3.43609 & 0.03475 & 14.19757 & 0.1064 & (14.13162, 14.26352) \\ \cline{2-13} 
 & 1450 & 3.43982 & 0.04531 & 3.64697 & 0.05972 & 3.67309 & 0.06887 & 3.45105 & 0.03251 & 14.21093 & 0.11033 & (14.14255, 14.27931) \\ \cline{2-13} 
 & 1500 & 3.43868 & 0.04281 & 3.64423 & 0.05926 & 3.66621 & 0.06579 & 3.45254 & 0.03632 & 14.20165 & 0.10245 & (14.13815, 14.26515) \\ \hline
\multirow{5}{*}{\textbf{FI-MAN}} & 1300 & 2.54791 & 0.20794 & 2.65836 & 0.20287 & 2.6082 & 0.23439 & 2.53345 & 0.18467 & 10.34792 & 0.15244 & (10.25344, 10.4424) \\ \cline{2-13} 
 & 1350 & 2.54344 & 0.21028 & 2.65381 & 0.20572 & 2.60286 & 0.23298 & 2.52207 & 0.18558 & 10.32218 & 0.15505 & (10.22608, 10.41828) \\ \cline{2-13} 
 & 1400 & 2.54155 & 0.21266 & 2.64653 & 0.20495 & 2.59576 & 0.23407 & 2.51734 & 0.18906 & 10.30118 & 0.14983 & (10.20832, 10.39404) \\ \cline{2-13} 
 & 1450 & 2.53465 & 0.21594 & 2.639 & 0.20474 & 2.59131 & 0.23568 & 2.51458 & 0.18981 & 10.27953 & 0.14173 & (10.19169, 10.36737) \\ \cline{2-13} 
 & 1500 & 2.52701 & 0.21597 & 2.6347 & 0.20466 & 2.58671 & 0.23793 & 2.50791 & 0.19065 & 10.25633 & 0.14 & (10.16956, 10.3431) \\ \hline
\multirow{5}{*}{\textbf{AP-MAN}} & 1300 & 3.44527 & 0.04825 & 3.65926 & 0.05535 & 3.68223 & 0.07323 & 3.43824 & 0.03005 & 14.225 & 0.17367 & (14.11736, 14.33264) \\ \cline{2-13} 
 & 1350 & 3.44218 & 0.04623 & 3.65175 & 0.05112 & 3.69095 & 0.06297 & 3.43844 & 0.03374 & 14.22331 & 0.15367 & (14.12807, 14.31855) \\ \cline{2-13} 
 & 1400 & 3.45943 & 0.0434 & 3.65922 & 0.05224 & 3.68724 & 0.0603 & 3.44132 & 0.03359 & 14.24721 & 0.12805 & (14.16785, 14.32657) \\ \cline{2-13} 
 & 1450 & 3.45133 & 0.04471 & 3.65107 & 0.05745 & 3.70086 & 0.06615 & 3.45699 & 0.03269 & 14.26026 & 0.12776 & (14.18107, 14.33945) \\ \cline{2-13} 
 & 1500 & 3.45034 & 0.04221 & 3.64837 & 0.0559 & 3.69416 & 0.06289 & 3.45762 & 0.03585 & 14.25049 & 0.12013 & (14.17603, 14.32495) \\ \hline
\multirow{5}{*}{\textbf{FIAP-MAN}} & 1300 & 2.52467 & 0.06002 & 2.61151 & 0.04857 & 2.62906 & 0.03563 & 2.58236 & 0.03475 & 10.3476 & 0.20936 & (10.21784, 10.47736) \\ \cline{2-13} 
 & 1350 & 2.51976 & 0.0588 & 2.60456 & 0.04871 & 2.62032 & 0.03527 & 2.57075 & 0.03706 & 10.3154 & 0.21398 & (10.18278, 10.44802) \\ \cline{2-13} 
 & 1400 & 2.51844 & 0.0574 & 2.59574 & 0.04722 & 2.61241 & 0.03483 & 2.5673 & 0.03411 & 10.29388 & 0.21186 & (10.16257, 10.42519) \\ \cline{2-13} 
 & 1450 & 2.50999 & 0.05775 & 2.58904 & 0.04559 & 2.60688 & 0.03335 & 2.56723 & 0.03213 & 10.27313 & 0.20298 & (10.14732, 10.39894) \\ \cline{2-13} 
 & 1500 & 2.50286 & 0.05482 & 2.58485 & 0.04242 & 2.60087 & 0.03261 & 2.55988 & 0.03054 & 10.24845 & 0.19404 & (10.12818, 10.36872) \\ \hline
\end{tabular}
\caption{50K Pattern $2^{\prime}$. Each Light}
\label{table: 50K_each_light_pattern_2_prime}
\end{table}
\end{landscape}
